Noise-Agnostic Multitask Whisper Training for Reducing False Alarm Errors in Call-for-Help Detection

Keyword spotting is often implemented by keyword classifier to the encoder in acoustic models, enabling the classification of predefined or open vocabulary keywords. Although keyword spotting is a crucial task in various applications and can be extended to call-for-help detection in emergencies, however, the previous method often suffers from scalability limitations due to retraining required to introduce new keywords or adapt to changing contexts. We explore a simple yet effective approach that leverages off-the-shelf pretrained ASR models to address these challenges, especially in call-for-help detection scenarios. Furthermore, we observed a substantial increase in false alarms when deploying call-for-help detection system in real-world scenarios due to noise introduced by microphones or different environments. To address this, we propose a novel noise-agnostic multitask learning approach that integrates a noise classification head into the ASR encoder. Our method enhances the model's robustness to noisy environments, leading to a significant reduction in false alarms and improved overall call-for-help performance. Despite the added complexity of multitask learning, our approach is computationally efficient and provides a promising solution for call-for-help detection in real-world scenarios.

==> 2-Background.tex <==
\section{Related Works}
\label{sec:Pre}
Sainath \textit{et al.}~\cite{sainath2015convolutional} demonstrated that CNNs could be used effectively on resource-constrained devices, but these models struggle to scale to new keywords without retraining. Chen \textit{et al.}~\cite{chen2015query} employed LSTMs for query-by-example for better performance of KWS, but their approach is not inherently robust to noisy environments. On the other hand, such as few-shot learning introduced by Mazumder \textit{et al.}~\cite{mazumder2021few} and Awasthi \textit{et al.}~\cite{awasthi2021teaching}, have improved the scalability of KWS models by reducing the need for retraining when new keywords are introduced. However, these models still suffer from performance degradation in noisy environments, where background noise or microphone interference can lead to false alarms. In terms of open-vocabulary keyword spotting, Liu \textit{et al.}~\cite{liu2021rnn} proposed leveraging RNN-T model for generalizing KWS beyond a fixed vocabulary. While this improves flexibility, the system still struggles with noise robustness and increased false alarm rates when deployed in the wild. In the call-for-help detection study~\cite{chu2021call}, they utilized an LVCSR-KWS framework, which is complicated cascaded system compared to more recent and advanced ASR models.

%While significant progress has been made in KWS, several gaps remain between previous works and the current needs of real-world applications. Previous works based on CNNs and RNNs have shown great promise in detecting predefined keywords, but their scalability and noise robustness remain limited. Sainath \textit{et al.}~\cite{sainath2015convolutional} demonstrated that CNNs could be used effectively on resource-constrained devices, but these models struggle to scale to new keywords without retraining. Similarly, Chen \textit{et al.}~\cite{chen2015query} leveraged LSTMs for query-by-example KWS, but their approach is not inherently robust to noisy environments. On the other hand, such as few-shot learning introduced by Mazumder \textit{et al.}~\cite{mazumder2021few} and Awasthi \textit{et al.}~\cite{awasthi2021teaching}, have improved the scalability of KWS models by reducing the need for retraining when new keywords are introduced. However, these models still suffer from performance degradation in noisy, real-world environments, where background noise or microphone interference can lead to false alarms. In terms of open-vocabulary keyword spotting, Liu \textit{et al.}~\cite{liu2021rnn} proposed leveraging RNN-T model for generalizing KWS beyond a fixed vocabulary. While this improves flexibility, the system still struggles with noise robustness and increased false alarm rates when deployed in the wild. Additionally, multitask learning techniques, such as those proposed by Shin \textit{et al.}~\cite{shin2022learning}, have introduced audio-text alignment and noise-agnostic approach, but the added complexity often requires higher computational resources, which can be a challenge for real-time or on-device KWS systems.

Compared to previous studies, we address the above limitations by introducing a noise-agnostic multitask learning framework that incorporates noise classification into the Whisper~\cite{radford2023robust} model. Our approach not only enhances scalability by leveraging a pretrained ASR model but also significantly reduces false alarms in noisy environments.
